A Survey of Text Watermarking in the Era of Large Language Models

Text watermarking algorithms are crucial for protecting the copyright of textual content. Historically, their capabilities and application scenarios were limited. However, recent advancements in large language models (LLMs) have revolutionized these techniques. LLMs not only enhance text watermarking algorithms with their advanced abilities but also create a need for employing these algorithms to protect their own copyrights or prevent potential misuse. This paper conducts a comprehensive survey of the current state of text watermarking technology, covering four main aspects: (1) an overview and comparison of different text watermarking techniques; (2) evaluation methods for text watermarking algorithms, including their detectability, impact on text or LLM quality, robustness under target or untargeted attacks; (3) potential application scenarios for text watermarking technology; (4) current challenges and future directions for text watermarking. This survey aims to provide researchers with a thorough understanding of text watermarking technology in the era of LLM, thereby promoting its further advancement.

==> tables/downstream.tex <==
\begin{table}[t]
\captionsetup{justification=raggedright}
  \caption{The corresponding relationship between text watermarking algorithms/benchmarks and the downstream tasks they used for evaluation.}
  \centering
  \scriptsize
  \renewcommand{\arraystretch}{1.6} % 设置行高
  \begin{tabular}{c m{3.2cm} m{9cm}}
    \hline
    \adjustbox{valign=c}{\includegraphics[width=0.48cm, height=0.4cm]{figures/icon/machine translation.pdf}} & \adjustbox{valign=c}{Machine Translation} &  Unbiased Watermark\citep{hu2023unbiased}, DiPmark\citep{wu2023dipmark}, NS-Watermark\citep{takezawa2023necessary}, Unforgeable Watermark\citep{liu2023private}, WaterBench\citep{tu2023waterbench}\\
    \hline
    \adjustbox{valign=c}{\includegraphics[width=0.48cm, height=0.4cm]{figures/icon/sentiment classification.pdf}} & \adjustbox{valign=c}{Sentiment Classification} & Binary-encoding Lexical Substitution\citep{yang2023watermarking} \\
    \hline
    \adjustbox{valign=c}{\includegraphics[width=0.5cm, height=0.4cm]{figures/icon/knowledge understanding.pdf}} & \adjustbox{valign=c}{Knowledge Understanding} & WaterBench \citep{tu2023waterbench} \\
    \hline
    \adjustbox{valign=c}{\includegraphics[width=0.5cm, height=0.4cm]{figures/icon/code generation.pdf}} & \adjustbox{valign=c}{Code Generation} & CodeMark\citep{sun2023codemark}, CoProtector\citep{sun2022coprotector}, SWEET\citep{lee2023wrote}, WaterBench\citep{tu2023waterbench} \\
    \hline
    \adjustbox{valign=c}{\includegraphics[width=0.35cm, height=0.4cm]{figures/icon/text summarization.pdf}} & \adjustbox{valign=c}{Text Summarization} & Unbiased Watermark\citep{hu2023unbiased}, DiPmark\citep{wu2023dipmark}, WaterBench\citep{tu2023waterbench} \\
    \hline
    \adjustbox{valign=c}{\includegraphics[width=0.5cm, height=0.4cm]{figures/icon/story generation.pdf}} & \adjustbox{valign=c}{Story Generation} & Invisible Watermarking \citep{zhao2023protecting} \\
    \hline 
    \adjustbox{valign=c}{\includegraphics[width=0.5cm, height=0.4cm]{figures/icon/question answering.pdf}} & \adjustbox{valign=c}{Question Answering} & WaterBench\citep{tu2023waterbench} \\
    \hline 
    \adjustbox{valign=c}{\includegraphics[width=0.5cm, height=0.4cm]{figures/icon/instruct following.pdf}} & \adjustbox{valign=c}{Instruction Following} & WaterBench\citep{tu2023waterbench} \\
    \hline 
  \end{tabular}
  \label{tab:task_specified}
\end{table}

==> tables/metrics.tex <==
\begin{table}[t]
\caption{Evaluation perspectives and metrics for text watermarking.}
\centering
\resizebox{0.99\textwidth}{!}{
\begin{tabular}{cccc}
\toprule
 Perspective &  Description & \multicolumn{2}{c}{ Metrics / Attacks} \\ 
\midrule
 \multirow{2}{*}{\makecell[c]{Detectability \\ (Sec. \color{blue}\ref{sec:success}\color{black})}} &  \multirow{2}{*}{\makecell[l]{Measures the capability of  \\ detecting the watermark}} &  Zero-bit & Binary Classification Metrics (i.e. F1, FPR, FNR)\\
\cmidrule{3-4}
 & &  Multi-bit &  Bit Error Rate (BER), Bit Accuracy\\ 
\midrule
 \multirow{11}{*}{\makecell[c]{Text Quality \\ (Sec. \color{blue}\ref{sec:quality}\color{black})}} &   \multirow{11}{*}{\makecell[l]{Assesses the impact of \\ watermarking on text quality}} &  Perplexity &  PPL\\
\cmidrule{3-4}
& &  Semantic Score & \\
\cmidrule{3-4}
& &   \multirow{8}{*}{Task-specified Evaluation} &  Machine Translation \\
& & &  Sentiment Classification \\
& & &  Knowledge Understanding \\
& & &  Code Generation \\
& & &  Text Summarization \\
& & &  Story Generation \\
& & &  Question Answering \\
& & &  Instruction Following \\
\cmidrule{3-4}
& &  Text Diversity &  Log Diversity\\
\midrule
\multirow{11}{*}{\makecell[c]{Robustness \\ (Sec. \color{blue}\ref{sec:robust}\color{black})}} &   \multirow{11}{*}{\makecell[l]{Evaluates the resilience of the \\ watermark against removal attacks}} &  Character-level &  Homoglyph Substitution\\
\cmidrule{3-4}
& & \multirow{4}{*}{Word-level} & Word Insertion \\
& & & Word Deletion \\
& & & Word Replacement \\
& & & Emoji Attack \\
\cmidrule{3-4}
& & \multirow{6}{*}{Document-level} & Back-translation \\
& & & CWRA \\
& & & Syntax Transformation \\
& & & Paraphrasing \\
& & & Watermark Collision \\
& & & Copy-paste Attack \\
\midrule
\multirow{3}{*}{\makecell[c]{Stealing Resistance \\ (Sec. \color{blue}\ref{sec:unfor}\color{black})}} &   \multirow{3}{*}{\makecell[l]{Measures the difficulty for attackers to \\ discern the watermarking method}} &  \multirow{3}{*}{Cracking Attacks} &  Spoofing Attack\\
& & & SCTS \\
& & & MIP \\
\bottomrule
\end{tabular}
}
\label{tab:metrics}
\end{table}

==> tables/objectives.tex <==
\begin{table}[t]
\caption{Relationships between text watermarking algorithms covered in the survey and the evaluation metrics, featuring
the individual objectives each text watermarking algorithm aims to achieve. $\blacktriangle$ stands for basic objectives, \Large$\bullet$ \small stands for primary objectives,
and \Large$\circ$ \small stands for secondary objectives.}
\label{tab:method_and_evaluation_metrics}
\centering
\resizebox{0.99\textwidth}{!}{
\begin{tblr}{
  columns = {m, m, m, m, m, m, m, m},
  row{1} = {c},
  row{2} = {c},
  row{3} = {c},
  row{4} = {c},
  row{5} = {c},
  row{6} = {c},
  row{7} = {c},
  row{8} = {c},
  row{9} = {c},
  row{10} = {c},
  row{11} = {c},
  row{12} = {c},
  row{13} = {c},
  row{14} = {c},
  row{15} = {c},
  row{16} = {c},
  row{17} = {c},
  row{18} = {c},
  row{19} = {c},
  row{20} = {c},
  row{21} = {c},
  row{22} = {c},
  row{23} = {c},
  row{24} = {c},
  row{25} = {c},
  row{26} = {c},
  row{27} = {c},
  row{28} = {c},
  row{29} = {c},
  row{30} = {c},
  row{31} = {c},
  row{32} = {c},
  row{33} = {c},
  row{34} = {c},
  row{35} = {c},
  row{36} = {c},
  row{37} = {c},
  row{38} = {c},
  cell{1}{1} = {c=3}{},
  cell{2}{1} = {r=2}{},
  cell{2}{2} = {r=2}{},
  cell{2}{3} = {r=2}{},
  cell{2}{6} = {r=2}{},
  cell{2}{7} = {r=2}{},
  cell{2}{8} = {r=2}{},
  cell{1}{4} = {c=5}{},
  cell{2}{4} = {c=2}{},
  cell{4}{1} = {r=14}{},
  cell{18}{1} = {r=21}{},
  cell{4}{2} = {r=4}{},
  cell{8}{2} = {r=5}{},
  cell{13}{2} = {r=3}{},
  cell{16}{2} = {r=2}{},
  cell{18}{2} = {r=4}{},
  cell{22}{2} = {r=14}{},
  cell{36}{2} = {r=3}{},
  hline{1,4} = {-}{0.08em},
  hline{2,18,39} = {-}{},
  hline{8,13,16,22,36} = {2-8}{},
  hline{3} = {4-6}{}
}
\textbf{Text Watermarking Algorithms} & & & \textbf{Objectives} & & & &  \\
{\textbf{Watermarked} \\ \textbf{Object}} & \textbf{Category} & \textbf{Method} & \textbf{Success Rate} & & \textbf{Text Quality} & \textbf{Robustness} & \textbf{Unforgeability} \\
& & & \textbf{Detection Accuracy} & \textbf{Payload} & & & \\

{Existing Text \\ (\color{blue}{\cref{sec:existing}}\color{black})} & {Format-based \\ 
(\color{blue}\cref{sec:format}\color{black})}& Line/Word-Shift Coding \citep{brassil1995electronic} & $\blacktriangle$ & & \Large$\bullet$ &  & \\

& & UniSpach \citep{POR20121075} & $\blacktriangle$ & \Large$\bullet$ & \Large$\bullet$ & & \\ 

& & Unicode Homoglyph Substitution \citep{rizzo2016content}& $\blacktriangle$ & \Large$\bullet$ & \Large$\bullet$ & & \\

& & EasyMark \citep{sato2023embarrassingly}& $\blacktriangle$ & \Large$\bullet$ & \Large$\bullet$ & & \\

& {Lexical-based \\ (\color{blue}\cref{sec:lexical}\color{black})}& Equimark \citep{topkara2006hiding}& $\blacktriangle$ &  & \Large$\bullet$ & \Large$\circ$ & \\

& & DeepTextMark \citep{munyer2023deeptextmark}& $\blacktriangle$ &  & \Large$\bullet$ & \Large$\bullet$ & \\

& & Context-aware Lexical Substitution \citep{yang2022tracing} & $\blacktriangle$ & \Large$\circ$ & \Large$\bullet$ & \Large$\circ$ & \\

& &  Binary-encoding Lexical Substitution \citep{yang2023watermarking} & $\blacktriangle$ & & \Large$\circ$ & \Large$\circ$ & \\

& & Robust Multi-bit Watermark \citep{yoo2023robust}& $\blacktriangle$ & \Large$\circ$ & \Large$\circ$ & \Large$\bullet$ & \\

& {Syntatic-based \\ (\color{blue}\cref{sec:syntactic}\color{black})}& NLW \citep{atallah2001natural}& $\blacktriangle$  & & & \Large$\bullet$ & \\

& & WANE \citep{10.1145/1178766.1178777}& $\blacktriangle$  & \Large$\bullet$ & \Large$\circ$ & \Large$\bullet$ & \\

& & MA-NLW \citep{meral2009natural}& $\blacktriangle$  & \Large$\bullet$ & \Large$\circ$ & \Large$\circ$ & \\

& {Generation-based \\ (\color{blue} \cref{sec:generation}\color{black})}& AWT \citep{abdelnabi2021adversarial}& $\blacktriangle$  & & \Large$\bullet$ & \Large$\bullet$ & \\

& & REMARK-LLM \citep{zhang2023remark}& $\blacktriangle$ & \Large$\bullet$ & \Large$\circ$ & \Large$\circ$ & \\

{LLMs \\(\color{blue}\cref{sec:llm}\color{black})} & {Training Time \\ (\color{blue}\cref{sec:train-watermark}\color{black})}& Dataset Trigger \citep{liu2023watermarking}& $\blacktriangle$  & & \Large$\bullet$ & & \\

& & Clean-Label Backdoor Watermark \citep{tang2023did}& $\blacktriangle$ & & \Large$\bullet$ & & \\

& & Coprotector \citep{sun2022coprotector}& $\blacktriangle$  & & \Large$\bullet$ & & \\

& & CodeMark \citep{sun2023codemark}& $\blacktriangle$  & & \Large$\bullet$ & & \\

& {Logits Generation \\ (\color{blue}\cref{sec:logits-watermark}\color{black})}& KGW \citep{DBLP:conf/icml/KirchenbauerGWK23}& $\blacktriangle$  & & \Large$\bullet$ &  &  \\ 

& & SWEET \citep{lee2023wrote}& $\blacktriangle$  & & \Large$\bullet$ &  & \\

& & Unbiased Watermark \citep{hu2023unbiased}& $\blacktriangle$  & & \Large$\bullet$ & \Large$\circ$ & \Large$\bullet$\\

& & DiPmark \citep{wu2023dipmark}& $\blacktriangle$  & & \Large$\bullet$ & \Large$\circ$ & \Large$\bullet$\\

& & COLOR \citep{yoo2023advancing}& $\blacktriangle$ & \Large$\bullet$ & \Large$\circ$ & & \\

& & CTWL \citep{wang2023towards} & $\blacktriangle$  & \Large$\bullet$ & \Large$\bullet$ & \Large$\circ$ & \Large$\bullet$\\

& & ThreeBrick \citep{fernandez2023three} & $\blacktriangle$  &  &  & \Large$\circ$ & \\

& & Unigram Watermark \citep{zhao2023provable}& $\blacktriangle$  & &  & \Large$\bullet$ & \\

& & KGW-reliability \citep{kirchenbauer2023reliability}& $\blacktriangle$  & & & \Large$\bullet$ & \\

& & NS-Watermark \citep{takezawa2023necessary}& $\blacktriangle$  & & \Large$\bullet$ & \Large$\circ$ & \\

& & SIR \citep{liu2023semantic}& $\blacktriangle$  & & \Large$\circ$ & \Large$\bullet$ & \Large$\bullet$ \\

& & Unforgeable Watermark \citep{liu2023private}& $\blacktriangle$  & & \Large$\circ$ & \Large$\circ$ & \Large$\bullet$ \\

& & Publicly Detectable Watermark \citep{cryptoeprint:2023/1661}& $\blacktriangle$  & & \Large$\circ$& \Large$\circ$ & \Large$\bullet$ \\

& & Semantic-based Robust Watermark \citep{ren2023robust}& $\blacktriangle$  & & \Large$\circ$ & \Large$\bullet$ & \\

& {Token Sampling \\ (\color{blue}\cref{sec:token-watermark}\color{black})}& Undetectable Watermark \citep{christ2023undetectable}& $\blacktriangle$  &  & \Large$\bullet$ & \Large$\circ$ & \Large$\bullet$\\

& & Robust Distortion-free Watermark \citep{kuditipudi2023robust} & $\blacktriangle$ & & \Large$\bullet$ & \Large$\bullet$ & \Large$\bullet$\\

& & SemStamp \citep{hou2023semstamp} & $\blacktriangle$ & & \Large$\circ$ & \Large$\bullet$ & 
\end{tblr}
}
\end{table}
